Exploiting Group-level Behavior Pattern forSession-based Recommendation

Session-based recommendation (SBR) is a challenging task, which aims to predict users' future interests based on anonymous behavior sequences. Existing methods leverage powerful representation learning approaches to encode sessions into a low-dimensional space. However, despite such achievements, all the existing studies focus on the instance-level session learning, while neglecting the group-level users' preference, which is significant to model the users' behavior. To this end, we propose a novel Repeat-aware Neural Mechanism for Session-based Recommendation (RNMSR). In RNMSR, we propose to learn the user preference from both instance-level and group-level, respectively: (i) instance-level, which employs GNNs on a similarity-based item-pairwise session graph to capture the users' preference in instance-level. (ii) group-level, which converts sessions into group-level behavior patterns to model the group-level users' preference. In RNMSR, we combine instance-level user preference and group-level user preference to model the repeat consumption of users, \ie whether users take repeated consumption and which items are preferred by users. Extensive experiments are conducted on three real-world datasets, \ie Diginetica, Yoochoose, and Nowplaying, demonstrating that the proposed method consistently achieves state-of-the-art performance in all the tests.

==> Section/Conclusion.tex <==
\section{Conclusion}

%In this paper, we study the problem of session-based recommendation, which is a challenging but practical task yet.
%%
%We propose a novel architecture for session-based recommendation via leveraging repeated behavior patterns and long-term dependencies of items over sessions.
%%
%Specifically, we convert sessions into repeated behavior patterns with item frequency for predicting re-consumption actions,
%and build similarity-based session graphs based on long-term item dependencies
%for learning item representations more accurately.
%%
%Extensive experiments on two large-scale real world datasets,
%which demonstrate that the repeated behavior patterns are effective to improve the accuracy of predicting next re-consumption action,
%and the proposed method significantly outperforms nine baseline methods, indicating it can be effectively used to solve real-world session-based recommendation problems.

{\color{red}
In this paper, we study the problem of session-based recommendation, which is a challenging but practical task yet.
%
By introducing group-level behavior patterns into SBR, we present a new perspective to learn the group-level users' preference, which also enhances the interpretability of the model.
%
Moreover, a novel similarity-based item-pairwise session graph is built to capture the long-term dependencies.
%
Extensive experiments on two large-scale real world datasets,
which demonstrate that our proposed method can provide a higher quality recommendation list,
indicating it can be effectively used to solve real-world session-based recommendation problems. 
}

==> Section/group_pattern_example.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
	\centering
	\small
	\caption{Examples of the group-level behavior patterns on Yoochoose.}
	\label{tab:staticForPatterns}
	\subfloat[The proportion of the repeat consumption in the next action for sessions with varying group-level behavior patterns.] {
	    \label{tab:pattern_1}
		\begin{tabular}{l|r}
    	\toprule[1pt]
    		{ \text{Group-level behavior patterns} } & \text{Proportion}\\
    		\hline
    		\hline
    		{ 1 -> 2 -> 2 -> 3 -> 3 -> 2 }  & 93\% \\
    		{ 1 -> 2 -> 1 -> 3 -> 2 -> 1 }  & 80\% \\
    		{ 1 -> 2 -> 3 -> 1 -> 4 -> 3 }  & 76\% \\
    		{ 1 -> 2 -> 3 -> 4 -> 2 -> 4 }  & 73\% \\
    		{ 1 -> 2 -> 3 -> 2 -> 4 -> 5 }  & 35\% \\
    		{ 1 -> 2 -> 2 -> 3 -> 4 -> 5 }  & 32\% \\
    		{ 1 -> 2 -> 3 -> 4 -> 5 -> 6 }  & 22\% \\
    	\bottomrule[0.8pt]
        \end{tabular}
	}
    
	\subfloat[The proportion of repeated consumption for each item in the next action.] {
		\label{tab:pattern_2}
		\begin{tabular}{l|c|c|c|c|c|c}
    	\toprule[1pt]
    		\multirow{2}{*}{\text{Group-level behavior patterns}} & \multicolumn{6}{c}{Proportion} \\ \cline{2-7}
            & 1 & 2& 3& 4& 5& 6\\
    		\hline
    		\hline
    		{ 1 -> 2 -> 2 -> 3 -> 3 -> 2 }  & 6\% & 89\% & 5\% & / & / & / \\
    		{ 1 -> 2 -> 1 -> 3 -> 2 -> 1 }  & 28\% & 42\% & 30\% & / & / & / \\
    		{ 1 -> 2 -> 3 -> 1 -> 4 -> 3 }  & 36\% & 19\% & 27\% & 19\% & / & / \\
    		{ 1 -> 2 -> 3 -> 4 -> 2 -> 4 }  & 12\% & 38\% & 22\% & 28\% & / & / \\
    		{ 1 -> 2 -> 3 -> 2 -> 4 -> 5 }  & 14\% & 21\% & 13\% & 28\% & 24\% & / \\
    		{ 1 -> 2 -> 2 -> 3 -> 4 -> 5 }  & 14\% & 21\% & 12\% & 18\% & 35\% & / \\
    		{ 1 -> 2 -> 3 -> 4 -> 5 -> 6 }  & 14\% & 11\% & 11\% & 12\% & 22\% & 29\% \\
    	\bottomrule[0.8pt]
        \end{tabular}
	}
\end{table}

Table \ref{tab:staticForPatterns} shows the examples of the group-level behavior patterns on Yoochoose. Specifically, Table \ref{tab:pattern_1} presents the proportion of the repeat consumption in the next action for sessions with varying group-level behavior patterns. It can be observed, users with group-level behavior pattern $'1->2->2->3->3->2'$ and $'1->2->3->1->4->3'$ has a high probability of repeat consumption in the next action, while users with $'1->2->2->3->4->5'$ and $'1->2->3->4->5->6'$ are more inclined to explore new items. The huge difference in probability distribution (\eg $93\%$ and $22\%$) shows the potential of the group-level behavior patterns in modeling the repeat consumption of users. And Table \ref{tab:pattern_2} presents the proportion of repeated consumption for each item in the next action, where most of users with $'1->2->2->3->3->2'$ favor item $'2'$ in the next action and users with $'1->2->3->1->4->3'$ prefer item $'2'$ than item $'1'$ and $'3'$. The statistics show the group-level users' preference contained in the group-level behavior patterns, which is significant when modeling the behavior of users.

==> Section/group_pattern_example_v2.tex <==
\section{Example}





\setlength{\tabcolsep}{4pt}
\begin{table}[t]
	\centering
	\small
	\caption{Examples of the group-level behavior patterns on Yoochoose.}
	\label{tab:staticForPatterns}
	\subfloat[The proportion of the repeat consumption in the next action for sessions with varying group-level behavior patterns.] {
	    \label{tab:pattern_1}
		\begin{tabular}{l|r}
    	\toprule[1pt]
    		{ \textbf{Group-level behavior patterns} } & \textbf{Proportion}\\
    		\hline
    		\hline
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} }  & 93\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} }  & 80\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{C} }  & 76\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} }  & 73\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{F} }  & 35\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} }  & 32\% \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} $\rightarrow$ \textbf{F} }  & 22\% \\
    	\bottomrule[0.8pt]
        \end{tabular}
	}

	\subfloat[The proportion of repeated consumption for each item in the next action.] {
		\label{tab:pattern_2}
		\begin{tabular}{l|c|c|c|c|c|c}
    	\toprule[1pt]
    		\multirow{2}{*}{\textbf{Group-level Behavior patterns}} & \multicolumn{6}{c}{\textbf{Proportion}} \\ \cline{2-7}
            & \textbf{A} & \textbf{B}& \textbf{C}& \textbf{D}& \textbf{E}& \textbf{F}\\
    		\hline
    		\hline
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} }  & 6\% & 89\% & 5\% & / & / & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} }  & 28\% & 42\% & 30\% & / & / & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{C} }  & 36\% & 19\% & 27\% & 19\% & / & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} }  & 12\% & 38\% & 22\% & 28\% & / & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{F} }  & 14\% & 21\% & 13\% & 28\% & 24\% & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} }  & 14\% & 21\% & 12\% & 18\% & 35\% & / \\
    		{ \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} $\rightarrow$ \textbf{F} }  & 14\% & 11\% & 11\% & 12\% & 22\% & 29\% \\
    	\bottomrule[0.8pt]
        \end{tabular}
	}
\end{table}

Table \ref{tab:staticForPatterns} shows the examples of the group-level behavior patterns on Yoochoose. Specifically, Table \ref{tab:pattern_1} presents the proportion of the repeat consumption in the next action for sessions with varying group-level behavior patterns. It can be observed, users with group-level behavior pattern $'ABBCCB'$ and $'ABACBA'$ has a high probability of repeat consumption in the next action, while users with $'ABBCDE'$ and $'ABCDEF'$ are more inclined to explore new items. The huge difference in probability distribution (\eg $93\%$ and $22\%$) shows the potential of the group-level behavior patterns in modeling the repeat consumption of users. And Table \ref{tab:pattern_2} presents the proportion of repeated consumption for each item in the next action, where most of users with $'ABBCCB'$ favor item $'B'$ in the next action and users with $'ABCADC'$ prefer item $'B'$ than item $'A'$ and $'C'$, it shows that users with same group-level behavior patterns may
have common preferences. The statistics show the group-level users' preference contained in the group-level behavior patterns, which is significant when modeling the behavior of users. 

==> Section/group_pattern_example_v3.tex <==
\setlength{\tabcolsep}{1pt}
\begin{table}[!t]
	\centering
	\footnotesize
	\caption{Group-level behavior pattern probability distribution on \emph{Yoochoose}.}
	\label{tab:staticForPatterns}
		\begin{tabular}{l|cc|c|c|c|c|c|cc|c}
    	\toprule[1pt]
    		\multirow{2}{*}{\textbf{Group-level Behavior Pattern}} & & \multicolumn{7}{c}{\textbf{Repeated Item}} & & \textbf{New} \\ \cline{3-9}
            & & \textbf{A} & \textbf{B}& \textbf{C}& \textbf{D}& \textbf{E}& \textbf{F} & \textbf{Sum} & & \textbf{Item} \\
    		\hline
    		\hline
    		{\textbf{1:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} } &  & 5\% & 83\% & 5\% & / & / & / & 93\% & & 7\% \\
    		{\textbf{2:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{A} } & & 22\% & 34\% & 24\% & / & / & / & 80\% & & 20\%  \\
    		{\textbf{3:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{A} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{C} } & & 28\% & 14\% & 20\% & 14\% & / & / & 76\% & & 24\% \\
    		{\textbf{4:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} } & & 8\% & 28\% & 16\% & 21\% & / & / & 73\% & & 27\%\\
    		{\textbf{5:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{F} } & & 4\% & 8\% & 5\% & 10\% & 8\% & / & 35\% & & 65\% \\
    		{\textbf{6:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} } & & 4\% & 7\% & 3\% & 6\% & 12\% & / & 32\% & & 68\% \\
    		{\textbf{7:} \textbf{A} $\rightarrow$ \textbf{B} $\rightarrow$ \textbf{C} $\rightarrow$ \textbf{D} $\rightarrow$ \textbf{E} $\rightarrow$ \textbf{F} } & & 3\% & 2\% & 2\% & 3\% & 5\% & 7\% & 22\% & & 78\%\\
    	\bottomrule[0.8pt]
        \end{tabular}
\end{table}



